PHANGS-HST: Globular Cluster Systems in 17 Nearby Spiral Galaxies

We present new catalogs of likely globular clusters (GCs) in 17 nearby spiral galaxies studied as part of the PHANGS-HST Treasury Survey. The galaxies were imaged in five broad-band filters from the near-ultraviolet through the $I$ band. PHANGS-HST has produced catalogs of stellar clusters of all ages by selecting extended sources (from multiple concentration index measurements) followed by morphological classification (centrally concentrated and symmetric or asymmetric, multiple peaks, contaminant) by visually examining the V-band image and separately by a machine-learning algorithm which classified larger samples to reach fainter limits. From both cluster catalogs, we select an initial list of candidate GCs to have $B-V \geq 0.5$ and $V-I \geq 0.73$~mag, then remove likely contaminants (including reddened young clusters, background galaxies misclassified by the neural network, and chance superpositions/blends of stars) after a careful visual inspection. We find that $\approx86$ % of the color-selected candidates classified as spherically symmetric, and $\approx68$ of those classified as centrally concentrated but asymmetric are likely to be GCs. The luminosity functions of the GC candidates in 2 of our 17 galaxies, NGC 628 and NGC 3627, are atypical, and continue to rise at least 1~mag fainter than the expected turnover near $M_V \sim -7.4$. These faint candidate GCs have more extended spatial distributions than their bright counterparts, and may reside in the disk rather than the bulge/halo, similar to faint GCs previously discovered in M101. These faint clusters may be somewhat younger since the age-metallicity degeneracy makes it difficult to determine precise cluster ages from integrated colors once they reach $\approx1$~Gyr.

==> Authors.tex <==



Response to Reviewer:

Firstly, we would like to start by thanking the Reviewer for making time to read the manuscript and offering their feedback to help improve it.  We have addressed each comment as explained below and shown in bold face font in the manuscript.


Comment: In section 1, the source for the GCLF is given as Secker (1992) - totally legitimate. But, in figure 10, the authors plot the GCLF from Harris (1996); this is a plot of the Milky Way GC data in the Harris catalog updated version of 2010 but not a reanalysis of the work by Secker. Readers may justifiably wonder why the Secker paper is referenced for the GCLF properties, but the data plotted in Figure 10 are from Harris. I have looked for a clarification on this point in the text but cannot find any. Maybe I have missed it? In any event the reason for the two references here should be clearer. Also, Rejkuba (2012) presents a clear and more recent discussion of the GCLF as a distance indicator that is more recent and broader than the Jordan (2007) paper and should probably be included in the discussion in section 7.


Response: Good point.  To tie together the earlier Secker results for the MW GCLF and Harris’ modern dataset for the GCs, we now fit a Gaussian to the  luminosity function for the MW GCs in the Harris catalog (2010 Version), and find very similar results as Secker: peak of -7.30+/-0.12 mag (us) vs. -7.29 (Secker) and a FWHM of 1.20+/-0.08 mag (us) vs. 1.1+/-0.1 (Secker). This  fit and the results are now shown in the upper-left panel of Figure 10 panel, given in the caption and text. 

We have also  added a reference to Rejkuba 2012 in the discussion section.

Comment: The data in Table 1 include the galaxy distances which, according to the footnote, are based on RGB tip and Cepheids. However there is no information on which (one or both) was used in each case, and the distance uncertainties for each galaxy. Including such information would be of value to the reader. One issue here is that TRGB and Cepheid data come from different parts of the galaxy and Cepheid data are much more likely to be affected by reddening. Are the distances given for only one method or both? And are the values from the two methods essentially the same for all galaxies when available, or are there disagreements? This additional information would help the reader interpret the results, particularly for the GCLF.

Response: We now give additional information and a fuller summary of the distance estimates, which were carefully compiled by Anand et al 2021 and are based on a variety of methods. We have added two columns to Table 1, one with the method and another with the citation to the distance measurement.  We have also added the following text to Section 2.1 to explain how Anand et al. prioritized available distance estimates.

“Distance determinations are from the compilation in \citet{Anand21}, and are based on a variety of methods.  Anand21 determined new distances to four of the galaxies based on the tip of the red giant branch (TRGB). For the rest, they carefully assessed distance estimates in the literature, which can vary in quality. They gave the highest preference to measurements based on the TRGB method and Cepheid variable.  The next preference was for standard candle methods, such as the planetary nebula luminosity function (PNLF), surface brightness fluctations.  When no distance estimates based on stellar populations were available, modeling methods were used to infer distance, either from numberical modeling of their orbits within a group or from the Numerical Action Method model of \citet{Shaya17}, which is a non-linear model that attempts to reconstruct the 3D orbits of galaxies.”

Comment: Section 3.2: Was the visual inspection by Whitmore done more than once? Cross checking can be invaluable in this type of work. If not more than once, are the authors confident that such issues as unconscious changing of criteria during the process are unimportant?

Response: The visual inspection specified in section 3.2 was not done by Whitmore, but Whitmore did assist by cross checking at many points in the creation process of the catalogs. Since a second independent classifier was used to reduce any inspector specific bias, we are confident that issues like unconscious changing of criteria are kept to a minimum.

Comment: Table 4 and related discussion: would the authors care to include specific frequency estimates for the GCs?

Response: We are planning to calculate specific frequencies (and color distributions)  in an upcoming paper, and we now state this in the last line of the conclusion. 

Writing/Grammar:
• In the abstract (lines 35-36), I suggest some clearer wording: "we find that...spherically symmetric and 68%.... asymmetric sources are likely to be GCs" 
Done
• Line 92: "sample includes nearly half"? 
Done
• Section 2 (line 129): a total of 8 apertures was used -
We think the sentence is correct as written 
• Table 2 footnote: "Columns 3 and 4 give the number and percentage" 
Done
• Figure 6 caption: "The number contaminants is shown in red" 
Done
• Foreground discussion (line 361): Besides misclassification it is probable that we ..."; I think probable is slightly stronger wording and more appropriate? 
Done
• Next paragraph (line 366): I suggest "we have concluded that a number" 
Done
• Line 384: introduced a method to determine"; fix is an idiosyncratic word choice here I think. 
Done
• Line 440: "higher background level... makes it " 
Done

